Robust Sparse Voting

Many applications, such as content moderation and recommendation, require reviewing and scoring a large number of alternatives. Doing so robustly is however very challenging. Indeed, voters' inputs are inevitably sparse: most alternatives are only scored by a small fraction of voters. This sparsity amplifies the effects of biased voters introducing unfairness, and of malicious voters seeking to hack the voting process by reporting dishonest scores. We give a precise definition of the problem of robust sparse voting, highlight its underlying technical challenges, and present a novel voting mechanism addressing the problem. We prove that, using this mechanism, no voter can have more than a small parameterizable effect on each alternative's score; a property we call Lipschitz resilience. We also identify conditions of voters comparability under which any unanimous preferences can be recovered, even when each voter provides sparse scores, on a scale that is potentially very different from any other voter's score scale. Proving these properties required us to introduce, analyze and carefully compose novel aggregation primitives which could be of independent interest.

==> app-additional-rel-work.tex <==
\section{Additional related work}
\label{sec:additional-rel-work}

==> impossibility.tex <==















==> primitives.tex <==
\section{Regularized statistics primitives}
\label{sec:primitives}

In this section, we introduce regularized statistical operators which will serve as the key primitives to our sparse robust and scale-resilient vote.
Such operators are critical to protect ourselves against attacks by malicious voters who would like to manipulate the scores of alternatives that few other voters, if any, previously scored.



\subsection{The regularized weighted median}

A common operator in voting theory is the (weighted) median $\median{}$.
Given voting rights $\votingrights{\voter} \geq 0$ and scores $\voterscore{\voter} \in \setR \cup \set{-\infty,+\infty}$, for all voter $\voter \in [\VOTER]$,
the median $M \triangleq \median{} (\votingrights{\voter}, \voterscore{\voter}~|~\voter \in [\VOTER]) \in \setR$ must guarantee that the left and right voting rights are at most half of all voting rights,
i.e. $\sum_{\voter : \voterscore{\voter} < M} \votingrights{\voter} \leq \frac{1}{2} \sum_{\voter \in [\VOTER]} \votingrights{\voter} \geq \sum_{\voter : \voterscore{\voter} > M} \votingrights{\voter}$.
When the context is clear, we simply denote it $\median{} (\votingrights{}, \voterscore{})$
Note that the median may be ill-defined, as there may be multiple real numbers satisfying these properties.
In this case, we define $\median{} (\votingrights{}, \voterscore{})$ to be the one closest to zero, which can be easily proven to be unique.

Unfortunately, however, the median does not satisfy Byzantine resilience.
After all, if an alternative $\alternative$ has been scored by no one, and if its global score is the median of all reported voters' scores, then any Byzantine voter that scores this alternative has arbitrary control over its global score.
This is very undesirable, especially in the context of Tournesol~\cite{tournesol}.

To guarantee Byzantine resilience, we introduce the regularized weighted median, which is parameterized by an additional weight $\votingresilience > 0$.
Let us also introduce the notation $\absv{x - y} \triangleq - \varepsilon x$ for $y = \varepsilon \infty$, with $\varepsilon \in \set{-1,+1}$.
We define the regularized weighted median as follows:
\begin{equation}
\label{eq:regmedian}
  \qrmedian{\votingresilience} (\votingrights{}, \voterscore{}) \triangleq \argmin_{x \in \setR} ~ \frac{1}{2} \votingresilience x^2 + \sum_{\voter \in [\VOTER]} \votingrights{\voter} \absv{x - \voterscore{\voter}}.
\end{equation}

\ysf{Properties (iii)-(vi) are never used.}

\begin{proposition}
\label{prop:qrmed-properties}
The following properties hold:
\begin{enumerate}[label=(\roman*)]
    \item $\qrmedian{\votingresilience} (\votingrights{}, \voterscore{})$ is well-defined.
    \item The influence of a single voter $\voter$ on $\qrmedian{\votingresilience}$ is bounded by $\frac{\votingrights{\voter}}{\votingresilience}$. \label{prop:qrmed-resilience-property}
    \item $\qrmedian{\votingresilience} (\votingrights{}, \voterscore{})$ has the same sign as $\median(\votingrights{}, \voterscore{})$ and $\absv{\qrmedian{\votingresilience} (\votingrights{}, \voterscore{})} \leq \absv{\median(\votingrights{}, \voterscore{})}$.
    \item $\qrmedian{\votingresilience} (\votingrights{}, \voterscore{}) = \median(\votingrights{}, \voterscore{})$ if and only if $\median(\votingrights{}, \voterscore{})=0$ or there exists $\voter \in [\VOTER]$ such that $\voterscore{\voter} = \median(\votingrights{}, \voterscore{}) \neq 0$ and $ \votingresilience \leq \frac{\votingrights{\voter}+\sign(\median)(\votingrights{}^+-\votingrights{}^-)}{\absv{\median(\votingrights{}, \voterscore{})}}$, where $\votingrights{}^+ \triangleq \sum_{\substack{\voterbis \in [\VOTER] \\ \voterscore{\voterbis}>\median}}\votingrights{\voterbis}$ and $\votingrights{}^- \triangleq \sum_{\substack{\voterbis \in [\VOTER] \\ \voterscore{\voterbis}<\median}}\votingrights{\voterbis}$.
    
    \item For any $\alpha \in (0,1)$, let $\quantile{\alpha}(\votingrights{},\voterscore{})$ the $\alpha$-quantile defined as:
    \begin{equation}
        \quantile{\alpha}(\votingrights{},\voterscore{}) \triangleq \argmin_{x \in \setR} \left ( \sum_{\voter \in [\VOTER]} \votingrights{\voter}  \right ) \cdot (1 - 2 \alpha) x + \sum_{\voter \in [\VOTER]} \votingrights{\voter} \absv{x - \voterscore{\voter}}.
    \end{equation}
    
    For any $\epsilon \in (0,\frac{1}{2})$, let $\alpha \triangleq \frac{1}{2}-\sign(\median)\epsilon$. We have $\qrmedian{\votingresilience} (\votingrights{}, \voterscore{}) = \quantile{\alpha}(\votingrights{}, \voterscore{})$ if and only if $\quantile{\alpha}(\votingrights{}, \voterscore{})=\frac{\sign(\median)}{\votingresilience}\sum_{\voter \in [\VOTER]} \votingrights{\voter}$ or there exists $\voter \in [\VOTER]$ such that $\voterscore{\voter} = \quantile{\alpha}(\votingrights{}, \voterscore{})$ and $\quantile{\alpha}(\votingrights{}, \voterscore{}) \in \left [\frac{-\votingrights{\voter}+\sign(\median)(\votingrights{}^+-\votingrights{}^-)}{\votingresilience},\frac{\votingrights{\voter}+\sign(\median)(\votingrights{}^+-\votingrights{}^-)}{\votingresilience} \right ] $, where $\votingrights{}^+ \triangleq \sum_{\substack{\voterbis \in [\VOTER] \\ \voterscore{\voterbis}>\quantile{\alpha}}}\votingrights{\voterbis}$ and $\votingrights{}^- \triangleq \sum_{\substack{\voterbis \in [\VOTER] \\ \voterscore{\voterbis}<\quantile{\alpha}}}\votingrights{\voterbis}$.
    \item Moreover, we have $\qrmedian{\votingresilience} (\votingrights{}, \voterscore{}) \in \left [\quantile{\alpha}(\votingrights{}, \voterscore{}), \median{}(\votingrights{},\voterscore{})\right ]$ if and only if $\votingresilience \leq \frac{\votingrights{\voter}+\sign(\median)(\votingrights{}^+-\votingrights{}^-)}{\absv{\quantile{\alpha}(\votingrights{}, \voterscore{})}}$.
    \item For any $\xi \in \setR^\VOTER$, we have
    \begin{equation}
        \absv{\qrmedian{\votingresilience} (\votingrights{}, \voterscore{}+\xi) - \qrmedian{\votingresilience} (\votingrights{}, \voterscore{})}
        \leq \norm{\xi}{\infty}.
    \end{equation}
    \label{prop:qrmed-perturbation-property}
    

\end{enumerate}
\end{proposition}

\begin{proof}
  Left in Appendix.
\end{proof}

If $\qrmedian{\votingresilience} (\votingrights{}, \voterscore{}) = \median(\votingrights{}, \voterscore{})$, then we say that the score is \emph{unconstrained}. Otherwise, we say that it is \emph{constrained}. In particular, if $\qrmedian{\votingresilience} (\votingrights{}, \voterscore{}) \in \left [\quantile{\frac{1}{2}-\epsilon}(\votingrights{}, \voterscore{}), \quantile{\frac{1}{2}+\epsilon}(\votingrights{}, \voterscore{}) \right ]$, we say that the score is \emph{$\epsilon$-constrained}.


\subsection{Quadratically regularized median $\qrmedian{}$}

We start with a regularized mean estimator, which we call the \emph{quadratically regularized median} $\qrmedian{}$.
$\qrmedian{}$ is parameterized by a nonnegative regularizer $\votingresilience \geq 0$ and a default value $\defaultmedian \in \setR$.
Given voting rights $\votingrights{} \in \setR_+^\VOTER$, scores $\voterscore{} \in \setR^\VOTER$ and lower and upper uncertainties $\uncertainty{-}, \uncertainty{+} \in (\setR_+^* \cup \set{\infty})^\VOTER$,
the quadratically regularized median $\qrmedian{}$ is then defined as
\begin{equation}
\label{eq:regularized_median}
  \qrmedian{} (\votingrights{}, \voterscore{}, \uncertainty{-}, \uncertainty{+} | \votingresilience, \defaultmedian) \triangleq
  \argmin_{x \in \setR} ~ \frac{1}{2} \votingresilience (x-\defaultmedian)^2 + \sum_{\voter \in [\VOTER]} \votingrights{\voter} \huber{} (x - \voterscore{\voter} | \uncertainty{-}, \uncertainty{+}).
\end{equation}
Note that this is the minimization of a one-dimensional strongly convex function.
It can thus be achieved in quasi-linear time in $\VOTER$, e.g. through dichotomic search of a zero-derivative point.

\begin{conjecture}
\label{conj:rmed-properties}
The following properties hold:
\begin{enumerate}[label=(\roman*)]
    \item $\qrmedian{}$ is well-defined.
    \item The additive influence of a single voter $\voter$ on $\qrmedian{}$ is bounded by $\frac{\votingrights{\voter}}{\votingresilience}$.
    \item For $\defaultmedian = 0$, $\qrmedian{}$ has the same sign as \median{}
    and $\absv{\qrmedian{}} \leq \absv{\median{}}$.
    \item $\lim_{\uncertainty{} \rightarrow 0} \qrmedian{} (\votingrights{}, \voterscore{}, \uncertainty{} | \votingresilience, \defaultmedian) = \median(\votingrights{}, \voterscore{}, \uncertainty{})$ if and only if $\median(\votingrights{}, \voterscore{}, \uncertainty{}) = \defaultmedian$
    or there exists $\voter \in [\VOTER]$ such that $\voterscore{\voter} = \median(\votingrights{}, \voterscore{})$ and $\absv{\median(\votingrights{}, \voterscore{})} \leq \frac{\votingrights{\voter}}{\votingresilience}$.
    \item $\lim_{\votingresilience \rightarrow 0, \uncertainty{} \rightarrow 0} \qrmedian{} (\votingrights{}, \voterscore{}, \uncertainty{} | \votingresilience, 0) = \median(\votingrights{}, \voterscore{}, \uncertainty{})$.
\end{enumerate}
\end{conjecture}

In particular, the discrepancy $\absv{\qrmedian{} (\votingrights{}, \voterscore{}, \uncertainty{} | \votingresilience, 0) - \qrmedian{} (\votingrights{}, \voterscore{}, \uncertainty{}| 0, 0)}$ is a good indicator of how much the median is \emph{constrained} by the regularization.

==> theorems.tex <==
\section{Theorems}
\label{sec:theorems}

We prove that our algorithms are correct.

